After the Fix: Transfer of Corrected Agent Experience

Does repairing an episode make its experience a better memory for the next task? We transfer the same failed source before and after accepted repair to a fixed target, alongside independent execution. Our 3,300 runs cover 100 ThinkingBox pairs and the same 100 APEX pairs with and without source-state inheritance, under eleven conditions. ThinkingBox's Full/Skill/Hybrid correction gains are 44/29/32 percentage points, with corrected performance 25/22/18 points above independence; inference weakens at the task-family level. Yet 12 of Full's 15-point larger correction gap over Skill come from worse uncorrected performance, not better corrected memory. Moreover, 22 of Full's 46 upward transitions restore observed baseline success. Neither APEX regime establishes comparable aggregate correction benefits. Action evidence connects workflow gains with reusable obligations and convention conflicts with source-local choices. Text APEX's accepted execution reaches 52% versus its summary's 40%, without robust global/group-level superiority or an estab- lished advantage over independence. Smaller handoffs reduce input but increase calls. The value of repairing experience is therefore distinct from the value of reusing it: memory updates require both a previous-version reference and a fresh-start reference.

==> data/regime_pairing/all_rows.tex <==
B-only & 42 & 44 / 55.54 & 47 / 57.40\\
U-None & 37 & 45 / 54.79 & 45 / 53.50\\
U-Full & 23 & 42 / 54.00 & 45 / 55.83\\
U-Skill & 35 & 39 / 50.89 & 44 / 54.29\\
U-Hybrid & 28 & 41 / 53.11 & 48 / 56.80\\
C-None & 36 & 44 / 55.38 & 47 / 56.10\\
C-Full & 67 & 41 / 49.10 & 45 / 53.51\\
C-Skill & 64 & 42 / 52.56 & 45 / 54.65\\
C-Hybrid & 60 & 45 / 54.41 & 40 / 48.53\\
Summary & 56 & 40 / 49.65 & 40 / 49.92\\
Execution & 67 & 44 / 52.33 & 52 / 58.88\\


==> data/regime_pairing/domains_en.tex <==
Banking & 48 & -10.4 / -6.2 & +0.0 / -6.2 & +0.0 / -18.8 & +14.6 / +10.4\\
Law & 23 & +4.3 / +0.0 & +17.4 / +30.4 & +17.4 / +4.3 & -8.7 / +21.7\\
Consulting & 29 & +10.3 / +10.3 & -3.4 / -10.3 & +0.0 / +0.0 & -3.4 / +6.9\\


==> data/regime_pairing/overlap_rows.tex <==
Full & 8 & 10 & 2 & 2 & 0 & 0\\
Skill & 15 & 14 & 5 & 5 & 3 & 2\\
Hybrid & 12 & 5 & 2 & 4 & 4 & 0\\
Execution--Summary & 12 & 14 & 2 & 0 & 0 & 4\\


==> data/regime_pairing/relations_en.tex <==
Same-family & 42 & -4.8 / +0.0 & +7.1 / -7.1 & -2.4 / -9.5 & +2.4 / +14.3\\
Shared procedure & 26 & +0.0 / +0.0 & +0.0 / +19.2 & +19.2 / -3.8 & +3.8 / +3.8\\
Shared evidence & 20 & -5.0 / +5.0 & -5.0 / -5.0 & -5.0 / -5.0 & +15.0 / +15.0\\
Context only & 12 & +16.7 / -8.3 & +8.3 / +0.0 & +8.3 / -16.7 & -8.3 / +16.7\\


==> data/representation/interactions.tex <==
TB & Full--None & +45 & [27.8, 61.9] & 0.0352\\
TB & Skill--None & +30 & [11.2, 48.6] & 0.3945\\
TB & Hybrid--None & +33 & [14.9, 53.9] & 0.0623\\
TB & Skill--Full & -15 & [-28.7, -1.4] & 1.0000\\
TB & Hybrid--Full & -12 & [-22.6, 2.4] & 1.0000\\
TB & Hybrid--Skill & +3 & [-11.3, 21.4] & 1.0000\\
State & Full--None & +0 & [-9.6, 8.8] & 1.0000\\
State & Skill--None & +4 & [-5.8, 12.7] & 1.0000\\
State & Hybrid--None & +5 & [-6.4, 15.2] & 1.0000\\
State & Skill--Full & +4 & [-4.2, 10.6] & 1.0000\\
State & Hybrid--Full & +5 & [-8.0, 17.3] & 1.0000\\
State & Hybrid--Skill & +1 & [-12.1, 12.9] & 1.0000\\
Text & Full--None & -2 & [-10.1, 4.9] & 1.0000\\
Text & Skill--None & -1 & [-12.3, 12.5] & 1.0000\\
Text & Hybrid--None & -10 & [-20.0, 1.0] & 1.0000\\
Text & Skill--Full & +1 & [-13.0, 16.7] & 1.0000\\
Text & Hybrid--Full & -8 & [-18.9, 4.3] & 1.0000\\
Text & Hybrid--Skill & -9 & [-20.6, 2.2] & 1.0000\\


==> data/representation/primary_cluster.tex <==
TB & H1a-full & +44 & [25.3, 56.2] & 0.0054 & 0.0439 & 0.1235\\
TB & H1a-skill & +29 & [12.8, 40.0] & 0.0259 & 0.1812 & 0.4917\\
TB & H1a-hybrid & +32 & [19.3, 44.0] & 0.0049 & 0.0439 & 0.1172\\
TB & H1b-full & +25 & [12.9, 37.6] & 0.0078 & 0.0703 & 0.1719\\
TB & H1b-skill & +22 & [8.0, 39.0] & 0.0203 & 0.1418 & 0.4053\\
TB & H1b-hybrid & +18 & [6.5, 32.5] & 0.0137 & 0.1094 & 0.2871\\
TB & H2a & +11 & [1.3, 18.7] & 0.0859 & 0.4297 & 1.0000\\
TB & H2b & +0 & [-6.2, 6.1] & 1.0000 & 1.0000 & 1.0000\\
State & H1a-full & -1 & [-7.7, 5.3] & 1.0000 & 1.0000 & 1.0000\\
State & H1a-skill & +3 & [-5.1, 10.7] & 0.6367 & 1.0000 & 1.0000\\
State & H1a-hybrid & +4 & [-5.8, 13.5] & 0.5732 & 1.0000 & 1.0000\\
State & H1b-full & -3 & [-13.3, 5.6] & 0.6953 & 1.0000 & 1.0000\\
State & H1b-skill & -2 & [-10.4, 6.9] & 0.8281 & 1.0000 & 1.0000\\
State & H1b-hybrid & +1 & [-7.2, 9.8] & 1.0000 & 1.0000 & 1.0000\\
State & H2a & +4 & [-5.2, 13.3] & 0.6250 & 1.0000 & 1.0000\\
State & H2b & -3 & [-13.1, 6.4] & 0.7031 & 1.0000 & 1.0000\\
Text & H1a-full & +0 & [-7.4, 6.2] & 1.0000 & 1.0000 & 1.0000\\
Text & H1a-skill & +1 & [-9.8, 13.2] & 1.0000 & 1.0000 & 1.0000\\
Text & H1a-hybrid & -8 & [-16.7, 2.0] & 0.1915 & 1.0000 & 1.0000\\
Text & H1b-full & -2 & [-14.3, 9.5] & 0.8794 & 1.0000 & 1.0000\\
Text & H1b-skill & -2 & [-10.1, 7.4] & 0.8281 & 1.0000 & 1.0000\\
Text & H1b-hybrid & -7 & [-15.6, 2.2] & 0.2412 & 1.0000 & 1.0000\\
Text & H2a & +12 & [3.1, 22.4] & 0.0469 & 0.2812 & 0.8438\\
Text & H2b & -7 & [-19.8, 4.2] & 0.3613 & 1.0000 & 1.0000\\


==> data/representation/within_branch.tex <==
TB & U-F--U-N & 4/18 & -14 & [-27.2, -4.3] & 0.1433 & 0.7734\\
TB & U-S--U-N & 12/14 & -2 & [-10.8, 4.8] & 1.0000 & 1.0000\\
TB & U-H--U-N & 9/18 & -9 & [-25.4, 3.3] & 1.0000 & 1.0000\\
TB & U-S--U-F & 16/4 & +12 & [2.0, 22.9] & 0.3782 & 1.0000\\
TB & U-H--U-F & 10/5 & +5 & [-4.3, 12.9] & 1.0000 & 1.0000\\
TB & U-H--U-S & 8/15 & -7 & [-20.7, 3.6] & 1.0000 & 1.0000\\
TB & C-F--C-N & 35/4 & +31 & [17.7, 42.4] & <.0001 & 0.1709\\
TB & C-S--C-N & 34/6 & +28 & [12.4, 42.1] & 0.0003 & 0.6143\\
TB & C-H--C-N & 29/5 & +24 & [14.6, 32.5] & 0.0013 & 0.1230\\
TB & C-S--C-F & 10/13 & -3 & [-12.7, 7.5] & 1.0000 & 1.0000\\
TB & C-H--C-F & 5/12 & -7 & [-14.3, 3.0] & 1.0000 & 1.0000\\
TB & C-H--C-S & 13/17 & -4 & [-12.8, 6.8] & 1.0000 & 1.0000\\
State & U-F--U-N & 9/12 & -3 & [-12.7, 5.5] & 1.0000 & 1.0000\\
State & U-S--U-N & 9/15 & -6 & [-13.7, 2.1] & 1.0000 & 1.0000\\
State & U-H--U-N & 7/11 & -4 & [-10.5, 3.3] & 1.0000 & 1.0000\\
State & U-S--U-F & 12/15 & -3 & [-14.4, 8.5] & 1.0000 & 1.0000\\
State & U-H--U-F & 9/10 & -1 & [-9.8, 10.5] & 1.0000 & 1.0000\\
State & U-H--U-S & 11/9 & +2 & [-6.6, 10.8] & 1.0000 & 1.0000\\
State & C-F--C-N & 10/13 & -3 & [-14.1, 7.5] & 1.0000 & 1.0000\\
State & C-S--C-N & 9/11 & -2 & [-8.8, 4.7] & 1.0000 & 1.0000\\
State & C-H--C-N & 7/6 & +1 & [-6.0, 7.7] & 1.0000 & 1.0000\\
State & C-S--C-F & 12/11 & +1 & [-9.0, 11.7] & 1.0000 & 1.0000\\
State & C-H--C-F & 12/8 & +4 & [-8.2, 16.1] & 1.0000 & 1.0000\\
State & C-H--C-S & 9/6 & +3 & [-4.3, 9.7] & 1.0000 & 1.0000\\
Text & U-F--U-N & 10/10 & +0 & [-7.3, 7.4] & 1.0000 & 1.0000\\
Text & U-S--U-N & 11/12 & -1 & [-10.8, 7.1] & 1.0000 & 1.0000\\
Text & U-H--U-N & 11/8 & +3 & [-6.0, 11.7] & 1.0000 & 1.0000\\
Text & U-S--U-F & 11/12 & -1 & [-11.0, 8.0] & 1.0000 & 1.0000\\
Text & U-H--U-F & 13/10 & +3 & [-6.4, 12.5] & 1.0000 & 1.0000\\
Text & U-H--U-S & 9/5 & +4 & [-2.6, 10.8] & 1.0000 & 1.0000\\
Text & C-F--C-N & 9/11 & -2 & [-12.0, 7.1] & 1.0000 & 1.0000\\
Text & C-S--C-N & 10/12 & -2 & [-10.2, 6.6] & 1.0000 & 1.0000\\
Text & C-H--C-N & 5/12 & -7 & [-16.0, 2.0] & 1.0000 & 1.0000\\
Text & C-S--C-F & 12/12 & +0 & [-9.7, 10.8] & 1.0000 & 1.0000\\
Text & C-H--C-F & 4/9 & -5 & [-11.3, 2.2] & 1.0000 & 1.0000\\
Text & C-H--C-S & 7/12 & -5 & [-12.9, 2.4] & 1.0000 & 1.0000\\


==> data/validator_transition_rows.tex <==
U-Full to C-Full & 55 & 2 & 54 & 37 & 17 \\
U-Skill to C-Skill & 40 & 7 & 39 & 28 & 11 \\
U-Hybrid to C-Hybrid & 48 & 3 & 48 & 30 & 18 \\
Summary to Execution & 13 & 1 & 13 & 8 & 5 \\

